The iWildCam 2020 Competition Dataset

Camera traps enable the automatic collection of large quantities of image data. Biologists all over the world use camera traps to monitor animal populations. We have recently been making strides towards automatic species classification in camera trap images. However, as we try to expand the geographic scope of these models we are faced with an interesting question: how do we train models that perform well on new (unseen during training) camera trap locations? Can we leverage data from other modalities, such as citizen science data and remote sensing data? In order to tackle this problem, we have prepared a challenge where the training data and test data are from different cameras spread across the globe. For each camera, we provide a series of remote sensing imagery that is tied to the location of the camera. We also provide citizen science imagery from the set of species seen in our data. The challenge is to correctly classify species in the test camera traps.

==> authors.tex <==
Sara Beery*$^\dagger$, Elijah Cole*, Arvi Gjoka$^\dagger$\\
\begin{tabular}{ccc}
California Institute of Technology* & Google$^\dagger$ 

\end{tabular}
